The Architectural Implications of Facebook's DNN-based Personalized Recommendation

The widespread application of deep learning has changed the landscape of computation in the data center. In particular, personalized recommendation for content ranking is now largely accomplished leveraging deep neural networks. However, despite the importance of these models and the amount of compute cycles they consume, relatively little research attention has been devoted to systems for recommendation. To facilitate research and to advance the understanding of these workloads, this paper presents a set of real-world, production-scale DNNs for personalized recommendation coupled with relevant performance metrics for evaluation. In addition to releasing a set of open-source workloads, we conduct in-depth analysis that underpins future system design and optimization for at-scale recommendation: Inference latency varies by 60% across three Intel server generations, batching and co-location of inferences can drastically improve latency-bounded throughput, and the diverse composition of recommendation models leads to different optimization strategies.

==> analysis.tex <==



==> background_backup.tex <==
\section{Background}

In this section we provide an overview of recommendation models including the overall task of personalized recommendation, the architecture of at-scale recommendation models, and key distinguishing features of DNN-based recommendation models (i.e., embedding tables) in terms of compute density, storage capacity, and memory access patterns.

%\begin{itemize}
%\item Deep learning models have significant storage requirements. For example, SparseNN models have very large embedding tables, which consume many gigabytes of storage and will likely continue growing in size. Such large models may not fit into the memory of an individual device, whether CPU or accelerator, and will require model partitioning among multiple device memories. Partitioning will result in communication overhead when data is located in another device’s memory. A good graph-partitioning algorithm will try to capture the notion of locality to reduce this communication overhead (https://code.fb.com/data-center-engineering/accelerating-infrastructure/).

%\item With the proper model partitioning, we can run very large deep learning models. With SparseNN models, for example, if the memory capacity of a single node is not enough for a given model, we can further shard the model among two nodes, boosting the amount of memory available to the model. Those two nodes are connected via multi-host NICs, allowing for high-speed transactions. This will increase communication overhead, but we can leverage the fact that there is access variance across the many embedding tables and sort the tables accordingly.
%\item How do we map SparseNN onto Kings Canyon?
%\end{itemize}

\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{figs/SparseNN.pdf}
  \caption{Overall model-architecture for production-scale recommendation models. Inputs to the model are a collection of dense and sparse features. Sparse features, unique to recommendation models, are transformed to a dense representation using embedding tables, shown in blue. The number and size of embedding tables, number of sparse feature (ID) lookups per table, as well as the depth and width of Bottom-FC and Top-FC layers varies based on the use-case.}
  \label{fig:sparsenn}
\end{figure}


\subsection{Recommendation Task}
% What is the overall goal of recommendation at a high-level and some example use-cases. 
Personalized recommendation is the task of recommending new content  to users based on their preferences.
As web-based services become ubiquitous around the globe, personalized recommendation systems are being used in more and more scenarios such as ranking social media posts, shopping items, and video recommendation~\cite{youtube, netflix}. 
Central to these services is the ability to accurately and efficiently rank content based on users' preferences.
For instance, estimates show that up to 75\% of videos consumed on Netflix and 60\% of views on Youtube come from their recommendation systems~\cite{chui2018notes}.
%https://www.microsoft.com/en-us/research/lab/microsoft-research-asia/articles/personalized-recommendation-systems/
It is important to accurately model users' preferences based their previous interactions such as clicks on posts, ratings, and purchases. 





% Compared to CNNs and RNNs, recommendation is hard because it includes mdoel not only dense features but also sparse features. Sparsity arises from not all users interact with all available content.
% This results in significantly different model-architectures to learn and predict based on both types of parameters.
Building highly accurate personalized recommendation system poses unique challenges as user preferences and previous interaction with content are represented as both dense and \textit{sparse} features \cite{eisenman2018bandana,naumov2019dimensionality}.
For instance, inputs to DNNs used for image classification and speech recognition are image or audio samples, which are represented as dense matrices and vectors.
The dense matrices and vectors are processed by a series of FC, CNN, or RNN layers.
In contrast, inputs to recommendation systems represent interactions between any two general entities (i.e., user preferences for online videos).
These inupts are a mix of dense and sparse features.
For instnce, in the case of ranking videos (e.g., Netflix, Youtube), there may be tens of thousands of potential videos that have been seen by millions of viewers. 
However, individual users interact with only a handful of videos.
This makes interactions between users and videos is sparse.
%This is also true of recommendation systems more broadly - input features are both dense and sparse. 
Sparse features not only make training more challenging but also requires intrinsically different operations (e.g., embedding tables) which impose unique compute, storage capacity, and memory access patterns demands (see Section \ref{sec:recModels} for details).

%inputs images or audio samples  
%ized recommendation is a
%The task of personalized recommendation 
%The task of recommendation is made hard as user %preferences and interactions with previous content is sparse.
%For instance, for web-based service there may be X to Y relevant content items to serve.
%Previous approaches relied on X but were inefficient as they required manual feature extraction and could not be trained end-to-end in a single model.
%Neural network approaches enable end-to-end training based off of raw dense and sparse features.
\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{figs/op_motivation.pdf}
  \caption{Compared to FC and CNN layers, embedding table operations (SparseLengthsSum, SPS, in Caffe2), seen in recommendation systems, exhibit high LLC cache miss rate (left) and low compute density (right).}
  \label{fig:embtable}
\end{figure}


\subsection{Recommendation Models} \label{sec:recModels}
% Overall architecture of the model includes embedding tables, MLPs, etc.
Figure \ref{fig:sparsenn} shows the overall architecture of state-of-art DNNs for personalized recommendation models. 
The model comprises a variety of operations such as FC layers, embedding tables (which transform sparse inputs to dense representations), pooling, and non-linearities, such as ReLU.
At a high-level, dense and sparse input features are separately transformed using FC layers and embedding tables respectively. 
% Would be nice to have examples of what these dense and sparse features are. 
The outputs of these transformations are then combined and processed by a final set of FC layers.

\textbf{Execution Flow:} The inputs, for a single user and single post, to recommendation models are a set of dense and sparse features. 
The output is the predicted click-through-rate (CTR) of the user and post.
Dense features are first processed by a series of FC layers, shown as the Bottom-FCs in Figure \ref{fig:sparsenn}.
On the other hand, sparse input features, represented as multiple vectors of sparse IDs, must first be made dense.
While, each vector of sparse IDs can be transformed to dense vectors using FC layers, the compute demands would be significant.
Instead, we use embedding tables.
Each vector is paired with an embedding table, as shown in Figure \ref{fig:sparsenn}, and each sparse ID is used to look-up a unique row in the embedding table.
The rows of the embedding are then combined into a single vector, typically with a dimension of 32 or 64, using element-wise gather operations.
Finally, these vectors and the output of the Bottom-FC layers are concatenated, and processed by the Top-FC layers show in Figure \ref{fig:sparsenn}.
The output is a single value representing the predicted CTR of the user-post pair.


%In Caffe2, this is accomplished by the SparseLengthSum operator. 

\textbf{Processing multiple posts:} 
At the data center scale, recommendations for many users and posts must be ranked simultaneously. 
Thus, it is important to note that the vectors of sparse IDs shown in Figure \ref{fig:sparsenn} correspond to inputs for a single user and single post.
% The output of a model is CTR for a single user-ad interaction.
% Batching enables computing CTR of many ads at once. 
To compute the CTR of many user-post pairs at once, requests are batched to improve overall throughput in the data center.

The depth and width of FC layers, number and size of embedding tables, number of sparse IDs per input, and typical batch-sizes depend on the use case of the recommendation model.
See Section \ref{sec:SparseNNParams} for more details.
% The inputs to the model are dense and sparse features for a given user and post.
% sparse features are transformed to dense vectors via embedding tables.
% Flow of model (inputs, embedding tables, mlps, etc.)

\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{figs/recommendation_pipeline.pdf}
  \caption{Content for production-scale recommendation systems is ranked hierarchically in two steps: filtering and ranking. 
  Filtering reduces the number of total items to a smaller subset using lightweight machine learning techniques or smaller DNN-based recommendation models (RM1).
  Ranking performs finer grained ranking using larger DNN-based recommendation models (RM2 and RM3).}
  \label{fig:flow}

\end{figure}

\subsection{Embedding Tables}
% A key distinguishing feature of recommendation models are the embedding tables. They are different than FC and other layers because of their storage requirement and access pattern.
A key distinguishing feature of DNNs for recommendation systems, compared to CNNs and RNNs, is the use of embedding tables.
As shown in Figure \ref{fig:sparsenn}, embedding tables tables are used to transform sparse input features to dense ones.
The dense representations are subsequently processed by a series of more traditional DNN layers including, FC, pooling, and ReLu non-linearities.
However, the embedding tables impose unique challenges to efficient execution in terms of their large storage capacity, low compute density, and irregular memory access pattern.

\input{modelparams.tex}

% Memory requirement: individual table can range from 100s of MB to GBs large.
% There can be many embedding tables based per model depending on the use case (will be discussed later)
\textbf{Storage capacity} 
The size of a single embedding table seen in production-scale recommendation models varies from tens of MBs to several GBs.
Furthermore, the number of embedding tables varies from 4 to 40, depending on the particular use case of the recommendation model.
(See Section \ref{sec:SparseNNParams} for details).
In aggregate, embedding tables for a single recommendation model can consume up to \fixme{20}GB of memory.
% Currently HW accelerators for ML often times only consider on-chip storage.
Thus, systems running production-scale recommendation models require large, off-chip storage such as DRAM or dense non-volatile memory \cite{eisenman2018bandana}.
% Maybe add something about individual layers in typical CNNs and RNNs require MBs of data (in aggregate models can need 100s of MBs but there is usually sufficient re-use in a single layer to amortize those costs; especially in CNNs) 

% Access pattern: Sparse ids are irregular memory accesses. Also note that not the entire table is brought in per input request to be ranked.
\textbf{Compute density and memory access pattern}
As shown in Figure \ref{fig:embtable}, compared to typical FC and CNN layers, embedding tables exhibit low compute density and irregular memory access patterns.
Recall that the embedding table operation (implemented as the \textit{SparseLengthsSum} operator in Caffe2\cite{caffe2} in production-scale recommendation models) entails reading a small subset of rows in the embedding table, based on input sparse IDs, which are combined using element-wise sum.
While, the entire embedding talbe is not read for a given input, the accesses follow a highly irregular memory access pattern.
On a Intel Broadwell server, seen in production data centers, this results in a higher LLC cache miss rate.
For instance, Figure \ref{fig:embtable}(left) shows that a typical SparseLengthsSum operator in production-scale recommendation models has an LLC cache miss rate of 8 MPKI \cite{eisenman2018bandana}, compared to 0.2 MPKI and 0.06 MPKI in FC and CNN layers respectively. 
Furthermore, the element-wise sum is a low-compute intensity operation.
For instance, as shown in Figure \ref{fig:embtable}(right), SparseLengthsSum (SPS) has a a compute density of 0.25 FLOPS/Byte compared to 18 FLOPS/Byte and 141 FLOPS/Byte for FC and CNNs layers found in typical DNN.
Due to their highly irregular memory access pattern and low-compute density, improving the efficiency of embedding table operations requires unique solutions, compared to the software and hardware acceleration approaches applied to typical FC and CNN layers.

==> introduction.tex <==
\section{Introduction}


%\paragraph{AI; Little effort devoted to recommendation}
Over the past five years, the systems and computer architecture community has devoted significant effort to optimizing the performance, energy efficiency, and memory consumption of deep neural networks (DNNs).
The optimizations include both algorithmic (e.g., more efficient DNN architectures, reduced precision datatypes) and system (e.g., parallelizing training and inference, hardware accelerators) advancements.
These optimizations have been considered for a range of DNNs, used in image classifications, object detection/tracking, and natural language processing, including ones with fully-connected (FC), convolutional (CNN), and recurrent (RNN) layers.
However, relatively little effort has been devoted to studying deep neural networks for recommendation workloads.
% Online search, online ads, and content recommendation

%\paragraph{Application/Scale of Recommendation models}
An increasing number of workloads such as online ads \cite{Clark} and content recommendation \cite{covington}, are using DNNs.
As web-scale applications become more ubiquitous across the globe, the amount of compute and storage resources devoted to DNNs for training and performing inference on such recommendation workloads continues to grow.
In fact, in a large scale internet company, these models comprise over 95\% of the cycles devoted to AI workloads in the datacenter.

%\paragraph{Pose new challenges}
% TODO: Need some high-level discussion about what recommendation workloads are
[Need a few sentences on overall architecture of recommendation models]
Unlike DNNs based on FC, CNN, and RNN layers, recommendation workloads follow distinct model architectures that pose unique challenges that existing solutions for efficient DNN execution do not solve:

% Embedding tables are bad. Compression FC layers is not a solution.
\textbf{Memory requirements:}
First, the DNNs for recommendation workloads consume an order of magnitude more memory than CNNs and RNNs.
The memory for recommendation workloads is found mainly in embedding tables, which store vectors of learned features to represent users and content.
Typical models can have between 4 and 50 embedding tables, each of which can require from single to hundreds MBs of storage, in a single model, requiring off-chip DRAM storage.
Furthermore, the embedding tables are not accessed in a regular memory access pattern with a fixed stride, but rather with an irregular memory access pattern with few and sparse lookups.
% Define what sparse means?
Thus, in addition to requiring off-chip DRAM, existing solutions for compressed sparse storage do not scale to the irregular memory access pattern for embedding tables.

\begin{figure}[ht!]
  \centering
  \includegraphics[width=\columnwidth, height=3cm]{figs/motivation.pdf}
  \vspace{-2em}
  \caption{Currently available benchmarks for personalized recommendation are not representative of production-scale workloads in terms of overall execution time, nor breakdown of time spent in operators}
  \label{fig:motiv}
\end{figure}

% Fraction of time spent on FC vs. embedding tables is not uniform can shift so accelerating FC layers may not be a solution.
\textbf{Diversity in model architecture:}
Next, DNNs for recommendation workloads span a variety of model architectures in terms of number and size of embedding tables, and depth and width of FC layers.
While in all models at least 98\% of the learned parameters are found in the embedding tables, the breakdown of compute cycles significantly varies.
For instance, as shown in Figure \ref{fig:motivation}, FC layers in RM3 models account for 98\% of the compute cycles whereas RM1 FC layers comprise of 60\% of the compute cycles.
As a result, solutions to speed up end-to-end recommendation models must consider accelerating not only FC layers but also embedding tables, which have very different memory access and compute patterns.
(In contrast, the performance bottleneck in DNNs for image classification, object detection/tracking, or NLP is determined by a single layer type - CNN and RNN).

% Throughput and latency
\textbf{Datacenter scale execution:}
Lastly, recommendation models used for online ads and content ranking serve billions of requests in datacenters worldwide.
Thus, to maintain service level agreements, DNN inference for recommendation models must balance inference latency with throughput.
This is accomplished by batching tens of inputs per inference, and simultaneously co-locating many batched inferences on a single machine.
However, co-locating models on a single machine introduces performance variability due to contention for system resources, adding complexity to optimal scheduling policies.
(In contrast, previous work optimizing FC, CNN, and RNN inference run-times focuses on reducing either inference for a unit batch size or a single model per machine).

[Need to beef this up] In this work, we conduct a thorough performance analysis of production scale recommendation models used in a large internet company, Company X.
The performance analysis demonstrates the key memory and compute challenges associated with efficiently running state-of-the-art recommendation models.
The key contributions of this work include:
\begin{itemize}
  \item Thorough single-model performance analysis of a diverse set of
    production scale recommendation models that reveals how inference latency
    varies across different Intel server platforms (Haswell, Broadwell,
    Skylake) as well as the batching dimension.
  \item  Thorough performance analysis of production-scale recommendation
    models that reveals co-locating models on a single machine introduces
    significant performance variability at the operator and end-to-end model
    level. We show that server platforms with inclusive L2/L3 cache-hierarchies
    (i.e., Intel Haswell and Broadwell) are particularly susceptible to
    performance variability.
    \item An open-source benchmark that is validated with internal
      recommendation workloads and can be configured to study a diverse set of
      production-scale recommendation models.
\end{itemize}


==> introductionV1.tex <==
\section{Introduction}

Recommendation systems are consuming the majority of computation cycles for machine learning services in data centers
advertisement, feeds, plus many other use cases (video ranking ...)

Existing research has largely focused on performance analysis and optimization for standard types of neural networks [cite].
The typical optimization techniques proposed for classic DNNs cannot be directly applied to recommendation systems.
This is because the architecture of neural networks for recommendation systems is different, introducing unique memory and computation demands.

Furthermore, data sets and model architectures that are available are not representative of production systems and their behavior [cite]. For example, compared to production systems, the NCF workload from MLPerf has fewer embedding tables (4 in MLPerf vs up to 40 in production systems), smaller embedding tables (10s of MB in MLPerf vs. up to 1GB in production systems), over 20x fewer irregular accesses per embedding, and fewer and smaller FC layers (~64K in MLPerf vs. up to 1.28M in production systems).
[talk about how its insufficient]. [# of embedding tables and FCs from the existing texts.]
Figure 1


To bridge the gap, in this paper, we describe and provide a suite of DNN recommenders that are representative of production-scale workloads. This will be open-sourced. We describe key metrics that can be used to quantitatively evaluate the performance of recommendation workloads. Our in-depth analysis of the production-scale recommenders shed key insights for system architecture and microarchitecture designs:

\begin{itemize}
  \item The inference latency varies significantly across several generations of Intel server architectures (Haswell, Broadwell, Skylake) that co-exist in production data centers.  [For the three models, does the optimal Intel server change? If so, say it here]. This is because [memory capacity, SIMD instructions/SSE vs. AVX, cache architecture].
  \item To reduce TCO, a typical solution is to co-locate recommenders. This, however, can introduce significant single model latency degradation, reducing the number of posts that can be ranked without violating service-level agreement (For example, latency requirement for different inference requests in range). We characterize the tradeoff between TCO/server utilization/inference throughput and performance variability of recommender co-location in production systems. Processor architectures with an inclusive L2/L3 cache hierarchy (Haswell and Broadwell) are particularly susceptible to performance degradation due to co-location. This introduces additional scheduling optimization at the data center scale.
  \item Hyperthreading introduces additional performance variability at the expense of improved inference throughput. [Are we recommending to turn off hyperthreading?]
  \item Across inference, there is typically no reuse at the cache hierarchy for the large size embedding tables (some #s) but we do find locality for the weights (some #s).
  \item We describe production-scale recommender architectures in this paper and propose a collection of synthetic recommender models with synthetic data sets. We perform detailed validation experiments for the production and synthetic models to be open sourced, along with detailed performance analysis and architecture insights.
  \item The current practice of using latency for benchmarking inference performance is insufficient. At data center scale, metrics of throughput (proxy for utilization and TCO), 95/99 are more representative as they determines the number of posts that can be ranked given SLA requirements. % latency are more representative [why].
\end{itemize}



==> introduction_v1.tex <==
\section{Introduction}

Machine learning (ML) is used in many production-scale data center services.
As web-scale applications become more ubiquitous across the globe, 
an increasing amount of compute and storage resources are devoted to ML training and inference~\cite{chung2018serving, tpu, hazelwood2018applied}.
% Some interesting information about number or energy of AI inferences in the datacenter would be interesting here: 
% For instance, each day, Facebook's infrastructure must perform over 200 trillion predictions % ^^^ Can we use this? (BR)
% https://code.fb.com/data-center-engineering/accelerating-infrastructure/
Personalized recommendation is an important class of these services.
For instance, McKinsey and Tech Emergence estimates that recommendation systems are responsible for driving up to 35\%  of Amazon's revenue~\cite{chui2018notes}.
%https://www.microsoft.com/en-us/research/lab/microsoft-research-asia/articles/personalized-recommendation-systems/
% The statistics from studies by McKinsey and Tech Emergence bear this out: this type of recommendation system brought Amazon 35 percent of its revenue and 23.7 percent growth to BestBuy. Up to 75 percent of video consumption on Netflix comes from the recommendation system and 60 percent of views on YouTube come from their recommendation feature.
State-of-the-art recommendation systems are used broadly throughout the industry to predict rankings for news feed posts, advertisements, and entertainment content. 
% Something about personalized about users?
A majority (over \fixme{95}\%) of the ML computation cycles in data centers
are consumed by DNN-powered personalized recommendation use cases~\cite{}.

%\textcolor{blue}{Citations: Serving DNNs in Real Time at Datacenter Scale with Project Brainwave Chung et al.; Google TPU; Amazon?}

Over the past few years, the system and computer architecture community has devoted significant efforts to optimize the performance, energy efficiency, and memory consumption of DNNs. 
The optimization techniques include both
algorithmic innovations, such as more efficient DNN architectures~\cite{},
reduced precision variables~\cite{},
and system advancements, such as parallelizing training and inference
~\cite{} and application-specific accelerators~\cite{tpu, minerva, eyeriss, eie, cambricon-x}.
These solutions primarily target convolutional neural networks (CNNs) and recurrent neural networks (RNNs)~\cite{resnet, yolo, ds2, ds3}.
% Do we want to say standard here?
However, the proposed optimization techniques for CNNs and RNNs cannot be directly applied to DNN-based recommendation models, because their architecture is intrinsically different, introducing unique memory and computation demands.
Furthermore, due to the nature of recommendation use cases, limited knowledge is often available of the models and associated challenges for efficient execution.

\begin{figure}[t!]
  \centering
  \includegraphics[width=\columnwidth]{figs/motivation.pdf}
  \vspace{-1em}
  \caption{Production-scale recommendation systems have orders of magnitude longer inference latency, larger embedding tables (memory intensity) and FC layers (compute intensity). The parameters of three sample production systems (RM1, RM2, and RM3) are  normalized to MLPerf-NCF to highlight the gaps.}
  \label{fig:motiv}
  \vspace{-1em}
\end{figure}


Data sets and model architectures that are currently available are not representative of production systems in terms of their memory and compute behaviors. 
Figure \ref{fig:motiv} illustrates the gap between currently available recommendation benchmarks, i.e. the neural-collaborative filtering implementation in MLPerf (MLPerf-NCF)~\cite{mlperf}, and  three production-scale recommendation models, RM1, RM2, and RM3. 
Compared to MLPerf, the production-scale models have orders of magnitude longer inference latency.
This is a result of discrepancies in the size and scale of two important features of recommendation systems: embedding tables (memory intensive) and fully-connected layers (compute intensive).
For instance, MLPerf-NCF has up to 10$\times$ fewer embedding tables; each table in MLPerf-NCF consumes tens of MB of storage, whereas embedding tables in production models require up to a few GBs. 
%In addition, MLPerf-NCF incurs over 20$\times$ fewer irregular memory accesses to embedding tables and implements fewer and smaller fully-connected (FC) layers.
In addition, MLPerf-NCF implements fewer and smaller fully-connected (FC) layers.
% Altogether, this creates a large disparity between currently-available and production-scale recommendation workloads.
Therefore, insights and solutions derived for much smaller recommendation models may not be applicable to nor representative of production systems and solutions.

% We develop and open-source synthetic recommendation models to study detailed implications on systems and architecture.
% We then take a step further, to study how recommendation models are run in production-environments. We find that hyperthreading and different queuing model 

In this paper, we describe a suite of personalized recommendation systems that are representative of production-scale workloads. 
First, we identify quantitative metrics to evaluate the performance of recommendation workloads for production use-cases.
Next, we use a suite of synthetic recommendation models to conduct detailed performance analysis. 
Since ML inference in the datacenter is run on a heterogeneous set of CPUs~\cite{hazelwood2018applied}, we study tradeoffs of running recommendation models on Intel Haswell, Broadwell, and Skylake servers.
Finally, we study performance characteristics of running recommendation models in production-environments. 
%The architectural and microarchitectural insights from this analysis can be used to guide broader system and architecture designs and optimization for at-scale recommendation use cases. 
%For example, we find that, by taking advantage of the heterogeneity of server architectures present in data centers, the optimal execution platform for maximizing throughput, while meeting strict SLA latency requirements, varies.

The in-depth analysis of production-scale recommendation systems shed the following insights for system architecture and microarchitecture designs
%[\textcolor{blue}{update based on the takeaway messages}]:

\begin{itemize}
    % Should we profile FC or embedding tables? Not entirely sure how to do that..
  % \item Across inference, there is relatively little reuse at the cache hierarchy in high-end Intel servers for the large size embedding tables (some \#s) but significant locality for FC weights (some \#s). (Section X)

    %
  \item The current practice of using latency only for benchmarking inference performance is insufficient. 
  At the data center scale, the metric of system throughput 
  %(a proxy of utilization and TCO) 
  under a latency constraint is more representative. The latency-bounded throughput measure determines the number of posts that can be ranked given service level agreement (SLA) requirements. (Section~\ref{sec:SparseNNParams}) % latency are more representative [why].
    % Inference latency with batching.
    
  \item Inference latency varies across several generations of Intel server architectures (Haswell, Broadwell, Skylake) that co-exist in data centers.
    With unit batch size, inference latency is optimized with Broadwell machines due to higher operating frequencies.
    % This is because inference with unit batch size are memory bound and higher operating frequency on Broadwell machines reduces run-time.
    On the other hand, throughput, with larger batch sizes, is optimized with Skylake machines.
    This is because larger batch-sizes increase the compute density of the FC layers.
    Compared to AVX-2 instructions in Haswell and Boradwell, compute-intensive FC layers are more readily accelerated by AVX-512 instructions in Skylake machines. (Section~\ref{sec:single}).
    %unit batch size [memory capacity, SIMD instructions/SSE vs. AVX, cache architecture].

  \item To further improve throughput, a typical solution is to co-locate multiple recommendation models on a single machine. 
    This, however, can degrade single model latency, and thus reduce the overall throughput of the system.
    %reducing the number of posts that can be ranked without violating service-level agreement (For example, latency requirement for different inference requests in range).
    We characterize the tradeoff between system architecture and inference throughput of recommendation systems in production.
    Processor architectures with inclusive L2/L3 cache hierarchies (i.e., Haswell, Broadwell) are particularly susceptible to performance degradation due to co-location.
    This introduces additional scheduling optimization opportunities at the data center scale. (Section~\ref{sec:colocation}).
    % Something about production data showing high performance variability.
  %\item Hyperthreading introduces additional performance variability at the expense of improved inference throughput. [Are we recommending to turn off hyperthreading?]
    % Are/How are we going to validate  benchmarks if we are using DLRM itself?
    
      \item Across at-scale recommendation models and different server architectures, the fraction of time spent on compute intensive operations, like FC, varies from 95\% down to 30\%.
      Thus, existing solutions for accelerating FC layers only \cite{tpu, minerva, eie, cambricon-x} will translate to lower end-to-end model inference latency for recommendation systems with dense input features but not ones with more sparse input features (Section~\ref{sec:single}).
      %Provided the diversity of recommendation systems in the production environment %\textcolor{blue}{do we have the frequency breakdown for RM1,2,3 so we can use to justify, in order to achieve e.g. 90\% coverage, we have to optimize for all instead of RM3?}
\end{itemize}

\textbf{Open-source:} To facilitate future work on at-scale recommendation systems from the systems and computer architecture community, we plan to open-source a suite of synthetic models, representative of production use cases. %, with synthetic data sets.
Together with the detailed performance analysis performed in this paper, the open-source implementations can be used to study compute requirements, storage capacity, and memory access patterns in at-scale recommendation systems.

%\textcolor{\Maxim}{We describe production-scale recommendation systems in this paper and conduct detailed performance analysis with architectural insights.
%To facilitate future work on production-scale recommendation systems, we plan to \textbf{open-source} the suite of synthetic models and data sets used in this paper. 
%}

%\footnote{\textcolor{\Maxim}{We plan to open source the collection of developed recommendation models, representative of production use
%cases, with synthetic data sets, to accurately model compute and storage requirements, as well as, memory access patterns.}}


 %\textcolor{\Maxim}{We describe production-scale recommender architectures in this paper and propose a collection of synthetic recommender models with synthetic data sets.
% We perform detailed validation experiments for the production and synthetic models to be \textbf{open-sourced}, along with detailed performance analysis and architecture insights.}


==> releated_work_notes.tex <==
More generally, \cite{open-rec} evaluates the accuracy impact of incorporating MLPs, CNN, and RNNs layers into the NCF model.
However, production systems such as 
%implication of using a combination of CNN 
[3] Deep Neural Networks for YouTube Recommendations (https://static.googleusercontent.com/media/research.google.com/en//pubs/archive/45530.pdf)


[6] OpenRec: A Modular Framework for Extensible and Adaptable Recommendation
Algorithms (http://www.cs.cornell.edu/~ylongqi/paper/YangBGHE18.pdf)
\begin{itemize}
\item An open-source recommendation framework from Cornell and MIT. The target
use case for this is mainly evaluating different recommendation systems based
on accuracy. It's a very general framework that tries to incorporate using
recurrent networks, CNN, MLPs, etc. On the other hand our contribution is
studying how production recommendation systems look like and performance
analysis (following systems/computer architecture).
\end{itemize}


[1] Bandana: Using Non-volatile Memory for Storing Deep Learning Models (https://arxiv.org/abs/1811.05922)


[2]Deep Learning Inference in Facebook Data Centers: Characterization, Performance Optimizations and Hardware Implications (https://arxiv.org/abs/1811.09886)



\begin{itemize}
\item This paper discusses Google's approach to running neural networks for
Youtube recommendations. There are two types of models: Deep Candidate
Generation and Ranking. The former filters Youtube videos down to a few hundred
that are of interest to the user. The latter ranks them to show the user.
\item Deep candidate generation follows very much so the form of NCF and
RM (e.g., dense features, sparse features with embedding tables, and FC
layers). The ranking model is similar except that it adds a some element-wise
operations for the output of embedding tables and dense features (general form
is similar).
\item FC layers are similarly sized: 1024/512/256, etc.
\end{itemize}

